Revisiting Assumptions Ordering in CAR-Based Model Checking

Model checking is an automatic formal verification technique that is widely used in hardware verification. The state-of-the-art complete model-checking techniques, based on IC3/PDR and its general variant CAR, are based on computing symbolically sets of under - and over-approximating state sets (called frames) with multiple calls to a SAT solver. The performance of those techniques is sensitive to the order of the assumptions with which the SAT solver is invoked, because it affects the unsatisfiable cores - which the solver emits when the formula is unsatisfiable - that crucially affect the search process. This observation was previously published in [15], where two partial assumption ordering strategies, intersection and rotation were suggested (partial in the sense that they determine the order of only a subset of the literals). In this paper we extend and improve these strategies based on an analysis of the reason for their effectiveness. We prove that intersection is effective because of what we call locality of the cores, and our improved strategy is based on this observation. We conclude our paper with an extensive empirical evaluation of the various ordering techniques. One of our strategies, Hybrid-CAR, which switches between strategies at runtime, not only outperforms other, fixed ordering strategies, but also outperforms other state-of-the-art bug-finding algorithms such as ABC-BMC.

==> 5.1RQ1.tex <==
\subsection{Results}



\noindent\textbf{A1. \UC Length in Different Literal Ordering Strategies.} 



\begin{table}[!ht]
    \centering
    \renewcommand{\arraystretch}{1.4}
    \caption{Average \UC Length in Different Strategies \label{tab:UClen}}
    \begin{tabular}{c|c} \tline
        Strategy        & \UC Length Average    \\ \tline
        None            & 241.1                 \\ \hline
        Intersection    & 400.0                 \\ \hline
        Rotation        & 475.6                 \\ \hline
        Combination(I+R) & 493.8                 \\ \hline
        Local(2)        & 412.8                 \\ \hline
        Local(3)        & 448.6                 \\ \hline
        Local(4)        & 434.7                 \\ \hline
        Local(5)        & 413.7                 \\ \tline
        
\end{tabular}
\end{table}

As shown in Table \ref{tab:UClen}, the average length of \UC varies across different strategies. However, all approaches that undergo reordering, regardless of the method employed, result in a greater length of \UC compared to those that remain unaltered. This is different from the understanding in ~\cite{DLPVR19}, which attributes the effectiveness of the literal ordering strategies to their ability to `compress the \UC'. In reality, it is observed that in the \emph{Intersection} strategy, the occurrence of a subsequent \UC falling within the $iCube$ may lead to a `compression'(\cite{DLPVR19}), albeit infrequently. Conversely, since all algorithms endeavour to maintain a focused search direction, the remaining spurious states become increasingly isolated, resulting in a generally longer \UC.

This intuitive observation -- that the length of \UC is positively correlated with the degree of focus in the search direction -- effectively elucidates the variance observed across these strategies. As discussed in previous sections, the \emph{Rotation} strategy introduces more literals in $rCube$ than the $iCube$, enhancing search focus. Conversely, in the \emph{\local} approaches, the arrangement of the joint part with previous states preceding the $rCube$ diminishes the degree of focus.

\iffalse
Meanwhile, with an increased portion of prioritised literals, the subsumption rate-- representing the frequency with which the \UC falls within the set of prioritised literals --  significantly rises in the approaches proposed by ~\cite{DLPVR19}. As can be seen in Table \ref{tab:Subs}, the subsumption rate is only 13\% in \emph{Intersection} while it reaches 40\% in \emph{Rotation}. \footnote{It may be puzzling that the proportion of prioritised literals in \emph{Rotation} is different from that in \emph{Intersection + Rotation}, despite our inference that $iCube \in rCube$. This discrepancy is due to the change in the search trail.}  This can be seen as a measurement of the ability to `predict' the forthcoming \UC and consequently steer the searching direction. In this way, such approaches managed to accelerate convergence.

\begin{table}[!ht]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \caption{Subsumption Rate in Different Strategies \label{tab:Subs}}
    \begin{tabular}{c|c|c} \tline
        Strategy        & Subsumption Rate     & Prioritized Literals Portion \\ \tline
        None            & 0\%                   & 0\%                       \\ \hline
        Intersection    & 12.82\%               & 10.86\%                   \\ \hline
        Rotation        & 40.20\%               & 84.28\%                   \\ \hline
        Combination(I+R) & 37.33\%               & 84.48\%                   \\ \hline
        Local(2)        & 47.56\%               & 84.72\%                   \\ \hline
        Local(3)        & 54.29\%               & 84.93\%                   \\ \hline
        Local(4)        & 58.19\%               & 84.89\%                   \\ \hline
        Local(5)        & 61.78\%               & 85.00\%                   \\ \tline
        
\end{tabular}
\end{table}


Furthermore, with the \emph{\local} strategies, the subsumption rates are even higher, with minimal overhead. As evident from the table, a marginal augmentation in the number of prioritised literals could enable the \emph{\local} strategies to increase the subsumption rate to a great extent. This, in turn, leads to an increased number of solved cases, a point we shall delve into later.

\fi




